Very Special Relativity in Curved Space-Times

The generalization of Cohen and Glashow's Very Special Relativity to curved space-times is considered. Gauging the SIM(2) symmetry does not, in general, provide the coupling to the gravitational background. However, locally SIM(2) invariant Lagrangians can always be constructed. For space-times with SIM(2) holonomy, they describe chiral fermions propagating freely as massive particles.

==> biblio.tex <==
\providecommand{\href}[2]{#2}\begingroup\raggedright\begin{thebibliography}{1}

\bibitem{Cohen:2006ky}
A.~G. Cohen and S.~L. Glashow, {\it {Very special relativity}},  {\em Phys.
  Rev. Lett.} {\bf 97} (2006) 021601,
  [\href{http://arxiv.org/abs/hep-ph/0601236}{{\tt hep-ph/0601236}}].

\bibitem{Cohen:2006ir}
A.~G. Cohen and S.~L. Glashow, {\it {A Lorentz-violating origin of neutrino
  mass?}},  \href{http://arxiv.org/abs/hep-ph/0605036}{{\tt hep-ph/0605036}}.

\bibitem{Fan:2006nd}
J.~Fan, W.~D. Goldberger, and W.~Skiba, {\it {Spin dependent masses and Sim(2)
  symmetry}},  {\em Phys. Lett.} {\bf B649} (2007) 186--190,
  [\href{http://arxiv.org/abs/hep-ph/0611049}{{\tt hep-ph/0611049}}].

\bibitem{Cohen:2006sc}
A.~G. Cohen and D.~Z. Freedman, {\it {Sim(2) and SUSY}},  {\em JHEP} {\bf 07}
  (2007) 039, [\href{http://arxiv.org/abs/hep-th/0605172}{{\tt
  hep-th/0605172}}].

\bibitem{Lindstrom:2006xh}
U.~Lindstrom and M.~Rocek, {\it {SIM(2) and superspace}},
  \href{http://arxiv.org/abs/hep-th/0606093}{{\tt hep-th/0606093}}.

\bibitem{Gibbons:2007iu}
G.~W. Gibbons, J.~Gomis, and C.~N. Pope, {\it {General Very Special Relativity
  is Finsler Geometry}},  {\em Phys. Rev.} {\bf D76} (2007) 081701,
  [\href{http://arxiv.org/abs/0707.2174}{{\tt arXiv:0707.2174}}].

\bibitem{Alvarez:2008uy}
E.~Alvarez and R.~Vidal, {\it {Very Special (de Sitter) Relativity}},
  \href{http://arxiv.org/abs/0803.1949}{{\tt arXiv:0803.1949}}.

\bibitem{Gibbons:2007zu}
G.~W. Gibbons and C.~N. Pope, {\it {Time-Dependent Multi-Centre Solutions from
  New Metrics with Holonomy SIM(n-2)}},
  \href{http://arxiv.org/abs/0709.2440}{{\tt arXiv:0709.2440}}.

\end{thebibliography}\endgroup

